Finding the Missing Baryons Using CMB as a Backlight

We present a new method for detecting the missing baryons by generating a template for the kinematic Sunyaev-Zel'dovich effect. The template is computed from the product of a reconstructed velocity field with a galaxy field; we find that the combination of a galaxy redshift survey such as SDSS and a CMB survey such as ACT and PLANCK can detect the kSZ, and thus the ionized gas, at significant signal-to-noise. Unlike other techniques that look for hot gas or metals, this approach directly detects the electrons in the IGM through their signature on the CMB. The estimated signal-to-noise for detecting the galaxy-momentum kSZ cross-correlation is 4, 9, and 12 for ACT (with survey area of 2000 $\mathrm{deg}^2$) with SDSS-DR4, SDSS3 and ADEPT respectively. The estimated signal-to-noise for PLANCK with SDSS-DR4, SDSS3 and ADEPT is 11, 23, and 32. Our method provides a new mean for determining properties of the ionized gas in the Universe. We provide galaxy momentum templates constructed from Sloan Digital Sky Survey online at our website at http://www.astro.princeton.edu/~shirley/SZ/SZ.html. The predicted correlation coefficients are provided along with the momentum maps. One can download the momentum templates and cross-correlate directly with CMB maps from ACT and PLANCK to detect the missing baryons.

==> Makefile <==
FILE=ms
PAGE=4
MAG=-1

all:
	latex ${FILE}
#	bibtex ${FILE}.aux
#	bibtex ${FILE}
#	latex ${FILE}
#	dvips ${FILE}
	dvips ${FILE}.dvi -o ${FILE}.ps
	ps2pdf ${FILE}.ps
	cp ${FILE}.pdf ~shirley/WWW/public/


latex:
	latex ${FILE}
	latex ${FILE}
	
ps:
	dvips ${FILE}
	ghostview -bg white -fg black -page ${PAGE} -magstep ${MAG} ${FILE}.ps &

dvips:
	latex ${FILE}
	latex ${FILE}
	dvips ${FILE}

view:
	ghostview -bg white -fg black -page ${PAGE} -magstep ${MAG} ${FILE}.ps &

clean:
	\rm -f ${FILE}.aux ${FILE}.dvi ${FILE}.log 

